Detection and characterization of microseismic events from fiber-optic DAS data using deep learning

Microseismic analysis is a valuable tool for fracture characterization in the earth's subsurface. As distributed acoustic sensing (DAS) fibers are deployed at depth inside wells, they hold vast potential for high-resolution microseismic analysis. However, the accurate detection of microseismic signals in continuous DAS data is challenging and time-consuming. We design, train, and deploy a deep learning model to detect microseismic events in DAS data automatically. We create a curated dataset of nearly 7,000 manually-selected events and an equal number of background noise examples. We optimize the deep learning model's network architecture together with its training hyperparameters by Bayesian optimization. The trained model achieves an accuracy of 98.6% on our benchmark dataset and even detects low-amplitude events missed during manual labeling. Our methodology detects more than 100,000 events allowing the reconstruction of spatio-temporal fracture development far more accurately and efficiently than would have been feasible by traditional methods.

==> SRL - Microseismic event detection/output.tex <==
\begin{thebibliography}{}
\itemsep0pt

\bibitem[Abadi et~al., 2015]{tensorflow2015-whitepaper}
Abadi, M., A. Agarwal, P. Barham, E. Brevdo, Z. Chen, C. Citro, G.~S. Corrado,
  A. Davis, J. Dean, M. Devin, S. Ghemawat, I. Goodfellow, A. Harp, G. Irving,
  M. Isard, Y. Jia, R. Jozefowicz, L. Kaiser, M. Kudlur, J. Levenberg, D.
  Man\'{e}, R. Monga, S. Moore, D. Murray, C. Olah, M. Schuster, J. Shlens, B.
  Steiner, I. Sutskever, K. Talwar, P. Tucker, V. Vanhoucke, V. Vasudevan, F.
  Vi\'{e}gas, O. Vinyals, P. Warden, M. Wattenberg, M. Wicke, Y. Yu, and X.
  Zheng (2015).
\newblock {TensorFlow}: Large-scale machine learning on heterogeneous systems.
\newblock (Software available from tensorflow.org).

\bibitem[Baird et~al., 2020]{Baird2020}
Baird, A.~F., A.~L. Stork, S.~A. Horne, G. Naldrett, J.-M. Kendall, J. Wookey,
  J.~P. Verdon, and A. Clarke (2020).
\newblock {Characteristics of microseismic data recorded by distributed
  acoustic sensing systems in anisotropic media}, {\em Geophysics} {\bf 85}
  KS139--KS147.

\bibitem[Bakku, 2015]{bakku2015fracture}
Bakku, S.~K. (2015).
\newblock {\em Fracture characterization from seismic measurements in a
  borehole}, PhD thesis, Massachusetts Institute of Technology.

\bibitem[Binder and Chakraborty, 2019]{Binder2019}
Binder, G., and D. Chakraborty (2019).
\newblock {Detecting microseismic events in downhole distributed acoustic
  sensing data using convolutional neural networks}, in {\em SEG Technical
  Program Expanded Abstracts 2019}, Society of Exploration Geophysicists,
  4864--4868.

\bibitem[Binder and Tura, 2020]{Binder2020}
Binder, G., and A. Tura (2020).
\newblock {Convolutional neural networks for automated microseismic detection
  in downhole distributed acoustic sensing data and comparison to a surface
  geophone array}, {\em Geophys. Prospect.} {\bf 68} 2770--2782.

\bibitem[Daley et~al., 2013]{daley2013field}
Daley, T.~M., B.~M. Freifeld, J. Ajo-Franklin, S. Dou, R. Pevzner, V.
  Shulakova, S. Kashikar, D.~E. Miller, J. Goetz, J. Henninges, et~al. (2013).
\newblock Field testing of fiber-optic distributed acoustic sensing (DAS) for
  subsurface seismic monitoring, {\em The Leading Edge} {\bf 32} 699--706.

\bibitem[Feurer et~al., 2019]{feurer2019auto}
Feurer, M., A. Klein, K. Eggensperger, J.~T. Springenberg, M. Blum, and F.
  Hutter (2019).
\newblock Auto-sklearn: efficient and robust automated machine learning, in
  {\em Automated Machine Learning}, Springer, Cham,  113--134.

\bibitem[Goodfellow et~al., 2016]{goodfellow2016deep}
Goodfellow, I., Y. Bengio, and A. Courville (2016).
\newblock {\em Deep learning}, MIT Press.

\bibitem[He et~al., 2015]{he2015deep}
He, K., X. Zhang, S. Ren, and J. Sun (2015).
\newblock Deep Residual Learning for Image Recognition, {\em arXiv preprint}
  1512.03385.

\bibitem[Huff et~al., 2020]{huff2020validating}
Huff, O., A. Lellouch, B. Luo, G. Jin, and B.~L. Biondi (2020).
\newblock Validating the origin of microseismic events in target reservoir
  using guided waves recorded by DAS, {\em The Leading Edge} {\bf 39} 776--784.

\bibitem[Huot and Biondi, 2018]{huot2018machine}
Huot, F., and B.~L. Biondi (2018).
\newblock Machine learning algorithms for automated seismic ambient noise
  processing applied to DAS acquisition, in {\em SEG Technical Program Expanded
  Abstracts 2018}, Society of Exploration Geophysicists,  5501--5505.

\bibitem[Huot and Biondi, 2020]{huot2020detecting}
--------, (2020).
\newblock Detecting earthquakes through telecom fiber using a convolutional
  neural network, in {\em SEG Technical Program Expanded Abstracts 2020},
  Society of Exploration Geophysicists,  3452--3456.

\bibitem[Huot et~al., 2018a]{huot2018jump}
Huot, F., B.~L. Biondi, and G. Beroza (2018a).
\newblock Jump-starting neural network training for seismic problems, in {\em
  SEG Technical Program Expanded Abstracts 2018}, Society of Exploration
  Geophysicists,  2191--2195.

\bibitem[Huot et~al., 2019]{huot2019automatic}
Huot, F., B.~L. Biondi, A. Lichnewsky, and C. Boneti (2019).
\newblock Automatic denoising by 2-D continuous wavelet transform, in {\em SEG
  Technical Program Expanded Abstracts 2019}, Society of Exploration
  Geophysicists,  3944--3948.

\bibitem[Huot et~al., 2021]{huot2021detecting}
Huot, F., A. Lellouch, P. Given, R.~G. Clapp, B.~L. Biondi, T. Nemeth, and K.
  Nihei (2021).
\newblock Detecting microseismic events on DAS fiber with super-human accuracy,
  Presented at the SEG/AAPG/SEPM First International Meeting for Applied
  Geoscience \& Energy, OnePetro.

\bibitem[Huot et~al., 2017]{huot2017automatic}
Huot, F., Y. Ma, R. Cieplicki, E.~R. Martin, and B. Biondi (2017).
\newblock Automatic noise exploration in urban areas, in {\em SEG Technical
  Program Expanded Abstracts 2017}, Society of Exploration Geophysicists,
  5027--5032.

\bibitem[Huot et~al., 2018b]{huot2018automated}
Huot, F., E.~R. Martin, and B. Biondi (2018b).
\newblock Automated ambient noise processing applied to fiber optic seismic
  acquisition (DAS), in {\em SEG Technical Program Expanded Abstracts 2018},
  Society of Exploration Geophysicists,  4688--4692.

\bibitem[IEA, 2019]{iea2019world}
IEA (2019).
\newblock {\em World Energy Outlook 2019}, IEA, Paris.

\bibitem[Ioffe and Szegedy, 2015]{ioffe2015batch}
Ioffe, S., and C. Szegedy (2015).
\newblock Batch normalization: Accelerating deep network training by reducing
  internal covariate shift, in {\em International conference on machine
  learning},  448--456.

\bibitem[Karrenbach et~al., 2019]{Karrenbach2019}
Karrenbach, M., S. Cole, A. Ridge, K. Boone, D. Kahn, J. Rich, K. Silver, and
  D. Langton (2019).
\newblock {Fiber-optic distributed acoustic sensing of microseismicity, strain
  and temperature during hydraulic fracturing}, {\em Geophysics} {\bf 84}
  D11--D23.

\bibitem[Kingma and Ba, 2014]{kingma2014adam}
Kingma, D.~P., and J. Ba (2014).
\newblock Adam: A method for stochastic optimization, {\em arXiv preprint}
  1412.6980.

\bibitem[Lal, 2004]{lal2004soil}
Lal, R. (2004).
\newblock Soil carbon sequestration to mitigate climate change, {\em Geoderma}
  {\bf 123} 1--22.

\bibitem[Lellouch et~al., 2021a]{lellouch2021properties}
Lellouch, A., E. Biondi, B.~L. Biondi, and M.~A. Meadows (2021a).
\newblock {Properties of a Deep Seismic Waveguide Measured With an Optical
  Fiber}, {\em Physical Review Research} {\bf 3} 13164.

\bibitem[Lellouch et~al., 2019]{lellouch2019observations}
Lellouch, A., S. Horne, M.~A. Meadows, S. Farris, T. Nemeth, and B.~L. Biondi
  (2019).
\newblock DAS observations and modeling of perforation-induced guided waves in
  a shale reservoir, {\em The Leading Edge} {\bf 38} 858--864.

\bibitem[Lellouch et~al., 2020a]{lellouch2020comparison}
Lellouch, A., N.~J. Lindsey, W.~L. Ellsworth, and B.~L. Biondi (2020a).
\newblock {Comparison between distributed acoustic sensing and geophones:
  Downhole microseismic monitoring of the FORGE geothermal experiment}, {\em
  Seismological Research Letters} {\bf 91} 3256--3268.

\bibitem[Lellouch et~al., 2020b]{Lellouch2020b}
Lellouch, A., M.~A. Meadows, T. Nemeth, and B.~L. Biondi (2020b).
\newblock {Fracture properties estimation using distributed acoustic sensing
  recording of guided waves in unconventional reservoirs}, {\em Geophysics}
  {\bf 85} M85--M95.

\bibitem[Lellouch et~al., 2021b]{lellouch2021low}
Lellouch, A., R. Schultz, N.~J. Lindsey, B.~L. Biondi, and W.~L. Ellsworth
  (2021b).
\newblock Low-magnitude seismicity with a downhole distributed acoustic sensing
  array—Examples from the FORGE geothermal experiment, {\em Journal of
  Geophysical Research: Solid Earth} {\bf 126} e2020JB020462.

\bibitem[Lellouch et~al., 2022]{lellouch2022microseismic}
Lellouch, L., B. Luo, F. Huot, R.~G.~C. Clapp, P. Given, E. Biondi, T. Nemeth,
  K.~T. Nihei, and B.~L. Biondi (2022).
\newblock Microseismic analysis over a single horizontal DAS fiber using guided
  waves, {\em Geophysics} .

\bibitem[Martin et~al., 2018]{martin2018seismic}
Martin, E.~R., F. Huot, Y. Ma, R. Cieplicki, S. Cole, M. Karrenbach, and B.~L.
  Biondi (2018).
\newblock A seismic shift in scalable acquisition demands new processing:
  Fiber-optic seismic signal retrieval in urban areas with unsupervised
  learning for coherent noise removal, {\em IEEE Signal Processing Magazine}
  {\bf 35} 31--40.

\bibitem[Metz et~al., 2005]{metz2005ipcc}
Metz, B., O. Davidson, H. De~Coninck, M. Loos, and L. Meyer (2005).
\newblock {\em IPCC special report on carbon dioxide capture and storage},
  Cambridge: Cambridge University Press.

\bibitem[Oldenburg et~al., 2009]{oldenburg2009certification}
Oldenburg, C.~M., S.~L. Bryant, and J.-P. Nicot (2009).
\newblock Certification framework based on effective trapping for geologic
  carbon sequestration, {\em International Journal of Greenhouse Gas Control}
  {\bf 3} 444--457.

\bibitem[Ramachandran et~al., 2017]{ramachandran2017searching}
Ramachandran, P., B. Zoph, and Q.~V. Le (2017).
\newblock Searching for activation functions, {\em arXiv preprint}  1710.05941.

\bibitem[Russakovsky et~al., 2015]{ILSVRC15}
Russakovsky, O., J. Deng, H. Su, J. Krause, S. Satheesh, S. Ma, Z. Huang, A.
  Karpathy, A. Khosla, M. Bernstein, A.~C. Berg, and L. Fei-Fei (2015).
\newblock {ImageNet Large Scale Visual Recognition Challenge}, {\em
  International Journal of Computer Vision (IJCV)} {\bf 115} 211--252.

\bibitem[Shere, 2013]{shere2013renewable}
Shere, J. (2013).
\newblock {\em Renewable: the world-changing power of alternative energy},
  Macmillan.

\bibitem[Simonyan and Zisserman, 2015]{simonyan2015deep}
Simonyan, K., and A. Zisserman (2015).
\newblock Very deep convolutional networks for large-scale image recognition,
  {\em arXiv preprint}  1409.1556.

\bibitem[Snoek et~al., 2012]{snoek2012practical}
Snoek, J., H. Larochelle, and R.~P. Adams (2012).
\newblock Practical bayesian optimization of machine learning algorithms, {\em
  Advances in neural information processing systems}  2951--2959.

\bibitem[Stork et~al., 2020]{Stork2020}
Stork, A.~L., A.~F. Baird, S.~A. Horne, G. Naldrett, S. Lapins, J.~M. Kendall,
  J. Wookey, J.~P. Verdon, A. Clarke, and A. Williams (2020).
\newblock {Application of machine learning to microseismic event detection in
  distributed acoustic sensing data}, {\em Geophysics} {\bf 85} KS149--KS160.

\bibitem[{The GPyOpt authors}, 2016]{gpyopt2016}
{The GPyOpt authors} (2016).
\newblock {GPyOpt}: A bayesian optimization framework in Python.

\bibitem[Verdon et~al., 2020]{Verdon2020}
Verdon, J.~P., S.~A. Horne, A. Clarke, A.~L. Stork, A.~F. Baird, and J.-M.
  Kendall (2020).
\newblock {Microseismic monitoring using a fibre-optic distributed acoustic
  sensor (DAS) array}, {\em Geophysics} {\bf 85} KS89--KS99.

\bibitem[Wilson and Gerard, 2007]{wilson2007carbon}
Wilson, E., and D. Gerard (2007).
\newblock {\em Carbon capture and sequestration: integrating technology,
  monitoring, regulation}, Blackwell Publishing, Ames, IA (United States).

\end{thebibliography}


==> output.tex <==
\begin{thebibliography}{}
\itemsep0pt

\bibitem[Abadi et~al., 2015]{tensorflow2015-whitepaper}
Abadi, M., A. Agarwal, P. Barham, E. Brevdo, Z. Chen, C. Citro, G.~S. Corrado,
  A. Davis, J. Dean, M. Devin, S. Ghemawat, I. Goodfellow, A. Harp, G. Irving,
  M. Isard, Y. Jia, R. Jozefowicz, L. Kaiser, M. Kudlur, J. Levenberg, D.
  Man\'{e}, R. Monga, S. Moore, D. Murray, C. Olah, M. Schuster, J. Shlens, B.
  Steiner, I. Sutskever, K. Talwar, P. Tucker, V. Vanhoucke, V. Vasudevan, F.
  Vi\'{e}gas, O. Vinyals, P. Warden, M. Wattenberg, M. Wicke, Y. Yu, and X.
  Zheng (2015).
\newblock {TensorFlow}: Large-scale machine learning on heterogeneous systems.
\newblock (Software available from tensorflow.org).

\bibitem[Baird et~al., 2020]{Baird2020}
Baird, A.~F., A.~L. Stork, S.~A. Horne, G. Naldrett, J.-M. Kendall, J. Wookey,
  J.~P. Verdon, and A. Clarke (2020).
\newblock {Characteristics of microseismic data recorded by distributed
  acoustic sensing systems in anisotropic media}, {\em Geophysics} {\bf 85}
  KS139--KS147.

\bibitem[Bakku, 2015]{bakku2015fracture}
Bakku, S.~K. (2015).
\newblock {\em Fracture characterization from seismic measurements in a
  borehole}, PhD thesis, Massachusetts Institute of Technology.

\bibitem[Binder and Chakraborty, 2019]{Binder2019}
Binder, G., and D. Chakraborty (2019).
\newblock {Detecting microseismic events in downhole distributed acoustic
  sensing data using convolutional neural networks}, in {\em SEG Technical
  Program Expanded Abstracts 2019}, Society of Exploration Geophysicists,
  4864--4868.

\bibitem[Binder and Tura, 2020]{Binder2020}
Binder, G., and A. Tura (2020).
\newblock {Convolutional neural networks for automated microseismic detection
  in downhole distributed acoustic sensing data and comparison to a surface
  geophone array}, {\em Geophys. Prospect.} {\bf 68} 2770--2782.

\bibitem[Daley et~al., 2013]{daley2013field}
Daley, T.~M., B.~M. Freifeld, J. Ajo-Franklin, S. Dou, R. Pevzner, V.
  Shulakova, S. Kashikar, D.~E. Miller, J. Goetz, J. Henninges, et~al. (2013).
\newblock Field testing of fiber-optic distributed acoustic sensing (DAS) for
  subsurface seismic monitoring, {\em The Leading Edge} {\bf 32} 699--706.

\bibitem[Feurer et~al., 2019]{feurer2019auto}
Feurer, M., A. Klein, K. Eggensperger, J.~T. Springenberg, M. Blum, and F.
  Hutter (2019).
\newblock Auto-sklearn: efficient and robust automated machine learning, in
  {\em Automated Machine Learning}, Springer, Cham,  113--134.

\bibitem[Goodfellow et~al., 2016]{goodfellow2016deep}
Goodfellow, I., Y. Bengio, and A. Courville (2016).
\newblock {\em Deep learning}, MIT Press.

\bibitem[He et~al., 2015]{he2015deep}
He, K., X. Zhang, S. Ren, and J. Sun (2015).
\newblock Deep Residual Learning for Image Recognition, {\em arXiv preprint}
  1512.03385.

\bibitem[Huff et~al., 2020]{huff2020validating}
Huff, O., A. Lellouch, B. Luo, G. Jin, and B.~L. Biondi (2020).
\newblock Validating the origin of microseismic events in target reservoir
  using guided waves recorded by DAS, {\em The Leading Edge} {\bf 39} 776--784.

\bibitem[Huot and Biondi, 2018]{huot2018machine}
Huot, F., and B.~L. Biondi (2018).
\newblock Machine learning algorithms for automated seismic ambient noise
  processing applied to DAS acquisition, in {\em SEG Technical Program Expanded
  Abstracts 2018}, Society of Exploration Geophysicists,  5501--5505.

\bibitem[Huot and Biondi, 2020]{huot2020detecting}
--------, (2020).
\newblock Detecting earthquakes through telecom fiber using a convolutional
  neural network, in {\em SEG Technical Program Expanded Abstracts 2020},
  Society of Exploration Geophysicists,  3452--3456.

\bibitem[Huot et~al., 2018a]{huot2018jump}
Huot, F., B.~L. Biondi, and G. Beroza (2018a).
\newblock Jump-starting neural network training for seismic problems, in {\em
  SEG Technical Program Expanded Abstracts 2018}, Society of Exploration
  Geophysicists,  2191--2195.

\bibitem[Huot et~al., 2019]{huot2019automatic}
Huot, F., B.~L. Biondi, A. Lichnewsky, and C. Boneti (2019).
\newblock Automatic denoising by 2-D continuous wavelet transform, in {\em SEG
  Technical Program Expanded Abstracts 2019}, Society of Exploration
  Geophysicists,  3944--3948.

\bibitem[Huot et~al., 2021]{huot2021detecting}
Huot, F., A. Lellouch, P. Given, R.~G. Clapp, B.~L. Biondi, T. Nemeth, and K.
  Nihei (2021).
\newblock Detecting microseismic events on DAS fiber with super-human accuracy,
  Presented at the SEG/AAPG/SEPM First International Meeting for Applied
  Geoscience \& Energy, OnePetro.

\bibitem[Huot et~al., 2017]{huot2017automatic}
Huot, F., Y. Ma, R. Cieplicki, E.~R. Martin, and B. Biondi (2017).
\newblock Automatic noise exploration in urban areas, in {\em SEG Technical
  Program Expanded Abstracts 2017}, Society of Exploration Geophysicists,
  5027--5032.

\bibitem[Huot et~al., 2018b]{huot2018automated}
Huot, F., E.~R. Martin, and B. Biondi (2018b).
\newblock Automated ambient noise processing applied to fiber optic seismic
  acquisition (DAS), in {\em SEG Technical Program Expanded Abstracts 2018},
  Society of Exploration Geophysicists,  4688--4692.

\bibitem[IEA, 2019]{iea2019world}
IEA (2019).
\newblock {\em World Energy Outlook 2019}, IEA, Paris.

\bibitem[Ioffe and Szegedy, 2015]{ioffe2015batch}
Ioffe, S., and C. Szegedy (2015).
\newblock Batch normalization: Accelerating deep network training by reducing
  internal covariate shift, in {\em International conference on machine
  learning},  448--456.

\bibitem[Karrenbach et~al., 2019]{Karrenbach2019}
Karrenbach, M., S. Cole, A. Ridge, K. Boone, D. Kahn, J. Rich, K. Silver, and
  D. Langton (2019).
\newblock {Fiber-optic distributed acoustic sensing of microseismicity, strain
  and temperature during hydraulic fracturing}, {\em Geophysics} {\bf 84}
  D11--D23.

\bibitem[Kingma and Ba, 2014]{kingma2014adam}
Kingma, D.~P., and J. Ba (2014).
\newblock Adam: A method for stochastic optimization, {\em arXiv preprint}
  1412.6980.

\bibitem[Lal, 2004]{lal2004soil}
Lal, R. (2004).
\newblock Soil carbon sequestration to mitigate climate change, {\em Geoderma}
  {\bf 123} 1--22.

\bibitem[Lellouch et~al., 2021a]{lellouch2021properties}
Lellouch, A., E. Biondi, B.~L. Biondi, and M.~A. Meadows (2021a).
\newblock {Properties of a Deep Seismic Waveguide Measured With an Optical
  Fiber}, {\em Physical Review Research} {\bf 3} 13164.

\bibitem[Lellouch et~al., 2019]{lellouch2019observations}
Lellouch, A., S. Horne, M.~A. Meadows, S. Farris, T. Nemeth, and B.~L. Biondi
  (2019).
\newblock DAS observations and modeling of perforation-induced guided waves in
  a shale reservoir, {\em The Leading Edge} {\bf 38} 858--864.

\bibitem[Lellouch et~al., 2020a]{lellouch2020comparison}
Lellouch, A., N.~J. Lindsey, W.~L. Ellsworth, and B.~L. Biondi (2020a).
\newblock {Comparison between distributed acoustic sensing and geophones:
  Downhole microseismic monitoring of the FORGE geothermal experiment}, {\em
  Seismological Research Letters} {\bf 91} 3256--3268.

\bibitem[Lellouch et~al., 2020b]{Lellouch2020b}
Lellouch, A., M.~A. Meadows, T. Nemeth, and B.~L. Biondi (2020b).
\newblock {Fracture properties estimation using distributed acoustic sensing
  recording of guided waves in unconventional reservoirs}, {\em Geophysics}
  {\bf 85} M85--M95.

\bibitem[Lellouch et~al., 2021b]{lellouch2021low}
Lellouch, A., R. Schultz, N.~J. Lindsey, B.~L. Biondi, and W.~L. Ellsworth
  (2021b).
\newblock Low-magnitude seismicity with a downhole distributed acoustic sensing
  array—Examples from the FORGE geothermal experiment, {\em Journal of
  Geophysical Research: Solid Earth} {\bf 126} e2020JB020462.

\bibitem[Lellouch et~al., 2022]{lellouch2022microseismic}
Lellouch, L., B. Luo, F. Huot, R.~G.~C. Clapp, P. Given, E. Biondi, T. Nemeth,
  K.~T. Nihei, and B.~L. Biondi (2022).
\newblock Microseismic analysis over a single horizontal DAS fiber using guided
  waves, {\em Geophysics} .

\bibitem[Martin et~al., 2018]{martin2018seismic}
Martin, E.~R., F. Huot, Y. Ma, R. Cieplicki, S. Cole, M. Karrenbach, and B.~L.
  Biondi (2018).
\newblock A seismic shift in scalable acquisition demands new processing:
  Fiber-optic seismic signal retrieval in urban areas with unsupervised
  learning for coherent noise removal, {\em IEEE Signal Processing Magazine}
  {\bf 35} 31--40.

\bibitem[Metz et~al., 2005]{metz2005ipcc}
Metz, B., O. Davidson, H. De~Coninck, M. Loos, and L. Meyer (2005).
\newblock {\em IPCC special report on carbon dioxide capture and storage},
  Cambridge: Cambridge University Press.

\bibitem[Oldenburg et~al., 2009]{oldenburg2009certification}
Oldenburg, C.~M., S.~L. Bryant, and J.-P. Nicot (2009).
\newblock Certification framework based on effective trapping for geologic
  carbon sequestration, {\em International Journal of Greenhouse Gas Control}
  {\bf 3} 444--457.

\bibitem[Ramachandran et~al., 2017]{ramachandran2017searching}
Ramachandran, P., B. Zoph, and Q.~V. Le (2017).
\newblock Searching for activation functions, {\em arXiv preprint}  1710.05941.

\bibitem[Russakovsky et~al., 2015]{ILSVRC15}
Russakovsky, O., J. Deng, H. Su, J. Krause, S. Satheesh, S. Ma, Z. Huang, A.
  Karpathy, A. Khosla, M. Bernstein, A.~C. Berg, and L. Fei-Fei (2015).
\newblock {ImageNet Large Scale Visual Recognition Challenge}, {\em
  International Journal of Computer Vision (IJCV)} {\bf 115} 211--252.

\bibitem[Shere, 2013]{shere2013renewable}
Shere, J. (2013).
\newblock {\em Renewable: the world-changing power of alternative energy},
  Macmillan.

\bibitem[Simonyan and Zisserman, 2015]{simonyan2015deep}
Simonyan, K., and A. Zisserman (2015).
\newblock Very deep convolutional networks for large-scale image recognition,
  {\em arXiv preprint}  1409.1556.

\bibitem[Snoek et~al., 2012]{snoek2012practical}
Snoek, J., H. Larochelle, and R.~P. Adams (2012).
\newblock Practical bayesian optimization of machine learning algorithms, {\em
  Advances in neural information processing systems}  2951--2959.

\bibitem[Stork et~al., 2020]{Stork2020}
Stork, A.~L., A.~F. Baird, S.~A. Horne, G. Naldrett, S. Lapins, J.~M. Kendall,
  J. Wookey, J.~P. Verdon, A. Clarke, and A. Williams (2020).
\newblock {Application of machine learning to microseismic event detection in
  distributed acoustic sensing data}, {\em Geophysics} {\bf 85} KS149--KS160.

\bibitem[{The GPyOpt authors}, 2016]{gpyopt2016}
{The GPyOpt authors} (2016).
\newblock {GPyOpt}: A bayesian optimization framework in Python.

\bibitem[Verdon et~al., 2020]{Verdon2020}
Verdon, J.~P., S.~A. Horne, A. Clarke, A.~L. Stork, A.~F. Baird, and J.-M.
  Kendall (2020).
\newblock {Microseismic monitoring using a fibre-optic distributed acoustic
  sensor (DAS) array}, {\em Geophysics} {\bf 85} KS89--KS99.

\bibitem[Wilson and Gerard, 2007]{wilson2007carbon}
Wilson, E., and D. Gerard (2007).
\newblock {\em Carbon capture and sequestration: integrating technology,
  monitoring, regulation}, Blackwell Publishing, Ames, IA (United States).

\end{thebibliography}

